End-to-End Information Extraction by Character-Level Embedding and Multi-Stage Attentional U-Net

Information extraction from document images has received a lot of attention recently, due to the need for digitizing a large volume of unstructured documents such as invoices, receipts, bank transfers, etc. In this paper, we propose a novel deep learning architecture for end-to-end information extraction on the 2D character-grid embedding of the document, namely the \textit{Multi-Stage Attentional U-Net}. To effectively capture the textual and spatial relations between 2D elements, our model leverages a specialized multi-stage encoder-decoders design, in conjunction with efficient uses of the self-attention mechanism and the box convolution. Experimental results on different datasets show that our model outperforms the baseline U-Net architecture by a large margin while using 40\% fewer parameters. Moreover, it also significantly improved the baseline in erroneous OCR and limited training data scenario, thus becomes practical for real-world applications.

==> background.tex <==
In this section, we provide a brief overview about the important components in our method: the 2D character-grid embedding and the box-convolutional network.

\subsection{2D character-grid embedding}
\input{background_chargrid.tex}
\subsection{Box-convolutional neural network}
\input{background_box_conv.tex}

==> background_box_conv.tex <==
\label{subsec:box_conv}
Box convolutions \cite{box_conv_Burkov2018} are sliding mean window with learnable offsets instead of weights over windows.
The intuitive display of the operation is included in Figure \ref{fig:box_convolution}.
\begin{figure}
    \centering
    \includegraphics[width=0.4\textwidth]{images/box_convolution.jpg}
    \caption{Box convolution operation, the output of the stored pixel value is calculated as the values of pixels covered by the box are accumulated according to the box cover ratio and taken mean w.r.t box area}
    \label{fig:box_convolution}
\end{figure}
Learning the offset aid the model in aggregating information from distanced regions in a straight forward way,
Making in a suitable alternative to spatial propagation network.
Further more, the box contribution can be weighted by applying a $1 \times 1$ convolution operations before and/or afterward and check the maximum absolute weight for each box-convoluted channels.

We utilize the box convolution as replacement for regular convolution layer in the encoders.

==> background_chargrid.tex <==
\label{subsec:chargrid}
Following \cite{Katti2018}, we represent composition input as a 2D character-grid (\textit{chargrid}), which in turn will be used as input to the segmentation module. Here, we give brief summary of the representation. Given the items:
\begin{itemize}
 \item A document image $I \in \left[0, 1\right]^{H \times W \times C}$ where $H$ and $W$ is the height and width of the document image respectively, $C$ is number of channels, typically 3.
 \item A set of $N$ text boxes in the document image $L=\{(t_1,b_1),(t_2,b_2),\ldots,(t_N,b_N)\}$ where $t_i$ is the text content of the $i$-th line and $b_i\in[0,1]^4$ denotes the normalized line position and size. This is the typical output of the text segmentation and OCR modules in a document processing pipeline. 
 \end{itemize}
 we can build the chargrid from character boxes, i.e., bounding boxes that each surround a single character somewhere on a given document page.  The coordinate space of a character box is defined by page height $H$ and width $W$ , and is usually measured in units of pixels.
\begin{figure}[h]
\centering
\includegraphics[width=0.35\textwidth]{chargrid}
\caption{Illustration of a chargrid representation}
\end{figure}

Intuitively, for each character $c_k$ at location $b_k$, the area covered by that character is filled with some constant index value $E(c_k)$. All remaining character-pixels corresponding to empty regions on the original document page are initialized with $0$. Figure 1 visualizes the chargrid representation of an example input document.
The reasons of which we adopt the chargrid are stated in \cite{Katti2018}, which we briefly summary below:
\begin{enumerate}
    \item All types of information can be unified (e.g text, font size, color, spatial position, table border, etc.). The chargrid can be down-sampled so that smallest component occupy one pixel in the smallest dimension, leading to optimized performance in segmentation.
    \item Chargrid also adds a certain degree of robustness against OCR and text-segmentation errors. We demonstrate this in figure \ref{fig:ocr_error} and figure \ref{fig:text_seg_error}.
\end{enumerate}
 
\begin{figure}[h]
\centering
\includegraphics[width=0.25\textwidth]{ocr_error}
\caption{Example of the mis-recognized character(s) in the OCR stage.}
\label{fig:ocr_error}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=0.25\textwidth]{text_seg_error}
\caption{The \textit{Over-split} and \textit{Over-merge} cases in the text segmentation stage.}
\label{fig:text_seg_error}
\end{figure}

We will now formulate the problem of information extraction as semantic segmentation on the 2D-character embedding of the document, which can be handled by a deep neural network, e.g. the fully convolutional network architecture we present in the next sub-sections. 

One final note is that before the chargrid representation is used as input to the deep neural network, we apply 1-hot encoding to the chargrid $g$. Thus, the original chargrid representation $g \in \mathbb{N}^{H \times W}$ becomes a vector representation $g \in \mathbb{R}^{H\times W\times N_C}$, where $N_C$ denotes the number of characters in the vocabulary including a padding/background character (in our case this is mapped to $0$) and an unknown character (all characters that are not mapped by our encoding $E$ will be mapped to this character).
